Experimental X-Ray Studies of Liquid Surfaces

Over the past two decades synchrotron facilities dedicated to the generation of x-rays for study of atoms, molecules and condensed matter have proliferated all over the world. As a result of the special properties of x-rays produced by these machines, there has been an enormous growth in the experimental possibilities. In this work we will demonstrate how these special properties can be used to carry out hitherto impossible measurements of the Angstrom level structure of the free surfaces of liquids. We demonstrate that surface structure of liquids is often different from that of the bulk. A large part of this thesis is devoted to surface-induced atomic or molecular layering phenomenon in metallic and dielectric liquids. In Chapters 1 through 10 we describe surface features of high-surface tension metals (Ga, In, Hg, Sn), as well as alkali metals (K, KNa) and water. The second part of the thesis (Chapters 11 through 16) is devoted to surface of binary metallic alloys (GaIn, HgAu, KNa, BiIn and GaBi), investigating a wide range of surface phenomena such as Gibbs adsorption and the tetra-point nanoscale wetting.

==> disclaimer.tex <==

%\section{Disclaimer for arXiv readers}
\refstepcounter{chapter} \addcontentsline{toc}{section}{Disclaimer
for arXiv readers}

\begin{center}

        \hyphenpenalty=10000\Large\expandafter\textbf\bf{Disclaimer for arXiv readers}
    \end{center}



This document describes work done by Oleg Shpyrko in fulfillment
of the requirements for the Ph.D. degree in the subject of Physics
at Physics Department, Harvard University.

\medskip

The version of thesis provided below has been modified for
electronic submission to arXiv.org. Most figures have been
reproduced using a lower resolution in order to adhere to space
requirements of \href

{http://www.arxiv.org}{arXiv} server.
However, a high-resolution
version of the thesis has also been made available at \\
\url{http://liquids.deas.harvard.edu/oleg/thesis/Thesis_all.pdf}

\medskip

Additionally, paper version of this dissertation submitted to the
Graduate School of Arts and Sciences omits some parts due to space
and format restrictions. The electronic version below provides all
of the omitted parts in full, in addition to extra features such
as hypertext citation, equation and figure referencing and keyword
indexing.

